Second-order mixed-moment model with differentiable ansatz function in slab geometry

We study differentiable mixed-moment models (full zeroth and first moment, half higher moments) for a Fokker-Planck equation in one space dimension. Mixed-moment minimum-entropy models are known to overcome the zero net-flux problem of full-moment minimum entropy $M_N$ models. Realizability theory for these modification of mixed moments is derived for second order. Numerical tests are performed with a kinetic first-order finite volume scheme and compared with $M_N$, classical $MM_N$ and a $P_N$ reference scheme.

==> Sections/scheme.tex <==
\section{Discontinuous-Galerkin scheme}

We consider a usual first-order system of hyperbolic balance laws
\begin{align}
\label{eq:GeneralHyperbolicSystem1D}
\dt\moments+\dz\Flux\left(\moments\right) = \Source\left(\moments\right),
\end{align}
where $\moments(\timevar,\x)\in\R^{\momentnumber}$ for all $\timevar\in\timeint$ and $\x\in\Domain$.

In the following, the spatial domain $\Domain = (\zL, \zR)$ is divided into (for notational simplicity) $\ncells$ (equidistant) cells $\cell{\cellind} = (\z_{\cellind-\frac12}, \z_{\cellind+\frac12})$, where the cell interfaces are given by $\z_{\cellind\pm\frac12} = \z_\cellind \pm 
\frac{\dzstepsize}{2}$ for cell centres $\z_\cellind = \zL + (\cellind - \frac12)\dzstepsize$, and
$\dzstepsize = \frac{\zR - \zL}{\ncells}$. 

Furthermore, $\SpaceOfPolynomials{\spatialorder}(\cell{\cellind})$ is the set of polynomials of degree at most $\spatialorder$ on the interval $\cell{\cellind}$, and 
\begin{equation}
\FiniteElementSpace{\spatialorder} = \{\Testfunction \in \Lp{1}(\Domain): \Testfunction|_{\cell{\cellind}} \in \SpaceOfPolynomials{\polydegree}(\cell{\cellind}) \text{ for } 
 \cellind \in \{ 1, \ldots , \ncells \} \}
\label{eq:dg-space}
\end{equation}
is the finite-element space of piecewise polynomials of degree $\polydegree$.\\

The discontinuous-Galerkin method for the general hyperbolic system \eqref{eq:GeneralHyperbolicSystem1D}, as outlined in \cite{Cockburn1989,Cockburn1989a,Cockburn1991}, can be briefly described as follows.

For each $\timevar\in\timeint$, seek an approximate solution $\momentsprojected(\timevar, \z)$ whose components live in the finite-element space $\FiniteElementSpace{\spatialorder}$ as defined in \eqref{eq:dg-space}.

Then follow the Galerkin approach: replace $\moments$ in \eqref{eq:GeneralHyperbolicSystem1D} by a 
solution of the form $\momentsprojected \in \FiniteElementSpace{\spatialorder}$, multiply the resulting equation by basis functions $\Testfunction[h]$ of $\FiniteElementSpace{\spatialorder}$ and integrate over cell $\cell{\cellind}$ to obtain
\begin{subequations}
\label{eq:dweakform1}
\begin{align}
 \dt \int_{\cell{\cellind}} \momentsprojected(\timevar, \z)\Testfunction[h](\z)~d\z
 &+ \Flux(\momentsprojected(\timevar, \z_{\cellind+\frac12}^-)) \Testfunction[h](\z_{\cellind+\frac12}^-)
  - \Flux(\momentsprojected(\timevar, \z_{\cellind-\frac12}^+)) \Testfunction[h](\z_{\cellind-\frac12}^+) \nonumber \\
 &-\int_{\cell{\cellind}} \Flux(\momentsprojected(\timevar, \z)) \dz \Testfunction[h](\z)~d\z 
 = \int_{\cell{\cellind}} \Source(\momentsprojected(\timevar, \z))\Testfunction[h](\z)~d\z  \label{eq:dweakform1a},\\
 \int_{\cell{\cellind}} \momentsprojected(0, \z)\Testfunction[h](\z)~d\z &= \int_{\cell{\cellind}} \momentstzero(\z) 
\Testfunction[h](\z)~d\z,
 \label{eq:dweakform1b}
\end{align}
\end{subequations}
where $\z_{\cellind \pm \frac12}^-$ and $\z_{\cellind \pm \frac12}^+$ again denote the limits 
from left and right, respectively, and $\momentstzero$ is the initial condition. 
In order to approximately solve the Riemann problem at the cell-interfaces,
the fluxes $\Flux(\momentsprojected(\timevar, \z_{\cellind + \frac12}^\pm))$ at the points of discontinuity are both replaced by a 
numerical flux $\numericalFlux(\momentsprojected(\timevar, \z_{\cellind+\frac12}^-), \momentsprojected(\timevar, \z_{\cellind+\frac12}^+))$, thus 
coupling the elements with their neighbours \cite{Toro2009}. Several well-known examples for such a numerical flux $\numericalFlux$ exist in literature. The simplest example is the global Lax-Friedrichs flux
\begin{align}
\label{eq:globalLF}
 \numericalFlux(\moments[1], \moments[2]) = \dfrac{1}{2} \left( \Flux(\moments[1]) + \Flux(\moments[2]) - C ( \moments[2] - 
 \moments[1]) \right).
\end{align}
The numerical viscosity constant $\viscosityconstant$ is taken as the global estimate of the 
absolute value of the largest eigenvalue of the Jacobian
$\Flux'$. 

The local Lax-Friedrichs flux could be used instead.
This requires computing the eigenvalues of the Jacobian in every
space-time cell to adjust the value of the numerical viscosity constant $\viscosityconstant$
but possibly decreases the overall diffusivity of the scheme.
However, since high-order methods are considered, the decrease in
diffusivity achieved by switching to the local Lax-Friedrichs flux should be
negligible.\\

The usual approach is to expand the approximate solution $\momentsprojected$ on each interval as
\begin{align}
\label{eqn:solution_form}
\left.\momentsprojected\right|_{\cell{\cellind}}(\timevar, \z) := \momentslocal{\cellind}(\timevar, \z) := \sum_{\polybasisind=0}^{\polydegree}\momentspolynomialcoefficients{\cellind}{\polybasisind}(\timevar) 
\Testfunction[\polybasisind]\left( \frac{\z - \z_\cellind}{\dzstepsize} \right),
\end{align}
where $\Testfunction[0], \Testfunction[1], \ldots ,\Testfunction[\polydegree]$ denote a 
basis for $\SpaceOfPolynomials{\spatialorder}(\referencecell)$ with respect to the standard $\Lp{2}$-scalar product on the reference cell $\referencecell = \left(-\frac12,\frac12\right)$. It is convenient to choose an orthogonal basis like the Legendre 
polynomials scaled to the interval $\referencecell$, denoted by
\begin{align}
\label{eq:LegendrePolynomialBasis}
\Testfunction[0](\referencevar) = 1, \quad \Testfunction[1](\referencevar) = 2\referencevar, \quad \Testfunction[2](\referencevar) = 
 \frac12 (12\referencevar^2-1), \: \ldots
\end{align}
With an orthogonal basis the cell means $\momentscellmean{\cellind}$ are easily available from the 
expansion coefficients $\momentspolynomialcoefficients{\cellind}{\polybasisind}$, since
$$
\momentscellmean{\cellind}(\timevar) := \frac{1}{\dzstepsize} \int_{\cell{\cellind}} \momentslocal{\cellind}(\timevar, \z)~d\z
 = \frac{1}{\dzstepsize} \sum_{\polybasisind=0}^{\polydegree} \momentspolynomialcoefficients{\cellind}{\polybasisind}(\timevar)
 \int_{\cell{\cellind}} \Testfunction[\polybasisind]\left( \frac{\z-\z_\cellind}{\dzstepsize} \right)~d\z
 = \momentspolynomialcoefficients{\cellind}{0}(\timevar).
$$
Collecting the coefficients $\momentspolynomialcoefficients{\cellind}{\polybasisind}(\timevar)$ into the $\spatialorder \times 
\momentnumber$ matrix
$$
\momentspolynomialmatrix{\cellind}(\timevar) = \left( \momentspolynomialcoefficients{\cellind}{0}(\timevar),\ldots , \momentspolynomialcoefficients{\cellind}{\polydegree}(\timevar)\right)^T,
$$

equation \eqref{eq:dweakform1} can be written in compact form as the coupled system of ordinary differential equations
\begin{align}
\label{eq:odeDG}
\dt \momentspolynomialmatrix{\cellind} &= \DifferentialOperatorLocal(\momentspolynomialmatrix{\cellind - 1}, \momentspolynomialmatrix{\cellind}, \momentspolynomialmatrix{\cellind + 1}), \quad 
\text{for } 
\cellind \in \{1, \ldots , \ncells\} \text{ and } \timevar \in \timeint,
\end{align}
with initial condition \eqref{eq:dweakform1b} and an appropriate choice of the local differential operator $\DifferentialOperatorLocal$.

We incorporate boundary conditions via `ghost cells' at $\z_0$ and $\z_{\ncells+1}$ and set $\momentslocal{0}(\timevar, \z)$ and $\momentslocal{\ncells + 1}(\timevar, \z)$ accordingly.

For Dirichlet-boundary conditions, the simplest approach is taken. The ghost-cell values are chosen to be the constant functions 
\begin{align*}
\momentslocal{0}(\timevar, \z) &\equiv \momentslocal{0}(\timevar, \z_{\frac12})\momentslocal{0}(\timevar, \z_{\frac12}),\\
\momentslocal{\ncells + 1}(\timevar, \z) &\equiv \momentslocal{\ncells + 1}(\timevar, \z_{\ncells + \frac12}),
\end{align*}
with $\momentslocal{0}(\timevar, \z_{\frac12})$ and $\momentslocal{\ncells + 1}(\timevar, \z_{\ncells + \frac12})$ defined by the boundary conditions.\\

For periodic boundary conditions, the obvious choice is
\begin{align*}
\momentslocal{0}(\timevar, \z) &= \momentslocal{\ncells}(\timevar, \z+\zR-\zL),\quad \z\in\cell{0},\\
\momentslocal{\ncells + 1}(\timevar, \z) &=\momentslocal{1}(\timevar, \z-\zR+\zL),\quad \z\in\cell{\ncells+1}.
\end{align*}

To obtain a high-order scheme for \eqref{eq:odeDG} a suitable time integrator has to be used. Such a class of integrators is given by the \emph{strong-stability-preserving} (\emph{SSP}) methods, as used for example in \cite{Zhang2010,AllHau12}. The
stages and steps of these type of methods are convex combinations of forward-Euler steps.
Since the realizable set is convex, the analysis of a forward-Euler step
then suffices to prove realizability preservation of the high-order method.\\

When possible, \emph{SSP-Runge-Kutta} (\emph{SSP-RK}) methods are used, but unfortunately they only exist up to order four \cite{Ruuth2004,Gottlieb2005}.
For higher orders the so-called \emph{two-step Runge-Kutta} (\emph{TSRK}) \emph{SSP}
methods \cite{Ketcheson2011} as well as their generalizations, the
\emph{multi-step Runge-Kutta} (\emph{MSRK}) \emph{SSP} methods \cite{Bresten2013} can be applied.
They combine Runge-Kutta schemes with positive weights and
high-order multistep methods to achieve a total order higher than
four while maintaining the important SSP property.

See \cite{Schneider2015b} for more information about the SSP-schemes used in the actual implementation. 

In this work we want to investigate different combinations of troubled-cell indicators $\tcindicator$ and slope limiters/reconstructors $\slopelimiter$.
In general, the process of limiting will be denoted by 

\begin{align}
\label{eq:slopelimiterscalar}
\momentspolynomialmatrix{\cellind} 
= 
\begin{cases}
\slopelimiter(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder})  & \text{ if } \tcindicator(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder}) = 1\\
\momentspolynomialmatrix{\cellind} & \text{otherwise}.
\end{cases}
\end{align}

It has been found that applying the limiter to the components 
themselves may introduce non-physical oscillations around an otherwise monotonic 
solution \cite{Cockburn1989}.
Instead, the limiter is applied to the local characteristic fields of the 
solution. They are found by transforming the vector $\moments$ 
using the matrix $\eigenvectormatrix_{\cellind}$, whose columns hold the eigenvectors of the Jacobian 
$\Flux'(\momentscellmean{\cellind})$ evaluated at the cell mean $\momentscellmean{\cellind}$.
After applying the limiter, the characteristic fields are transformed back to the conserved quantities.
In the end, since $\momentspolynomialmatrix{\cellind}$ is a matrix of size $\spatialorder \times \momentnumber$, this transformation is accomplished by post-multiplying with $\eigenvectormatrix_{\cellind}^{-T}$ 
so that
\begin{align}
\label{eq:DGLimiter}
 \slopelimitercf(\momentspolynomialmatrix{\cellind-1},\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+1}) = \slopelimiter(\momentspolynomialmatrix{\cellind-1}\eigenvectormatrix_{\cellind}^{-T},\momentspolynomialmatrix{\cellind}\eigenvectormatrix_{\cellind}^{-T},\momentspolynomialmatrix{\cellind+1}\eigenvectormatrix_{\cellind}^{-T})\eigenvectormatrix_{\cellind}^T,
\end{align}
and similarly for $\tcindicator$.

In the following we will neglect the transformation to characteristic fields for notational simplicity.

\subsection{WENO reconstruction and smoothness indicators}

\subsection{Troubled-cell indicators}
\comment{blabla}

\subsubsection{TVBM-corrected minmod indicator}
\label{sec:TVBMminmod}
An often-used indicator is the \emph{TVBM-corrected minmod limiter} proposed in
\cite{Cockburn1989a}. It assumes that the major part of the spurious oscillations is generated in the linear part of the underlying polynomial, whose slope in the reference cell is simply $\momentspolynomialcoefficients{\cellind}{1}$.

The indicator in the $\cellind^{\text{th}}$ cell is then given by
\begin{align}
\tcindicator(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder})
= 
\begin{cases}
1 & \text{ if }
     \abs{\momentspolynomialcoefficients{\cellind}{1}} \geq \TVBconstant(\dzstepsize)^2 \text{ and } \minmod{\momentspolynomialcoefficients{\cellind}{1}, \momentspolynomialcoefficients{\cellind+1}{0} - \momentspolynomialcoefficients{\cellind}{0}, 
                  \momentspolynomialcoefficients{\cellind}{0} - \momentspolynomialcoefficients{\cellind-1}{0}} \neq \momentspolynomialcoefficients{\cellind}{1},\\
0 &\text{otherwise}.                 
\end{cases}
% \slopelimiter(\momentspolynomialmatrix{\cellind-1},\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+1}) = \left\{ 
%  \begin{array}{cc}
%   \left( \begin{array}{c}
%           \left( \momentspolynomialcoefficients{\cellind}{0} \right)^T \\
%            \minmod{\momentspolynomialcoefficients{\cellind}{1}, \momentspolynomialcoefficients{\cellind+1}{0} - \momentspolynomialcoefficients{\cellind}{0}, 
%             \momentspolynomialcoefficients{\cellind}{0} - \momentspolynomialcoefficients{\cellind-1}{0}}^T \\
%           (0, 0, \ldots , 0)\\
%           \vdots\\
%           (0, 0, \ldots , 0)
%          \end{array} \right)
%    &\text{ if }
%     \abs{\momentspolynomialcoefficients{\cellind}{1}} \geq \TVBconstant(\dzstepsize)^2, \\     
%    \momentspolynomialmatrix{\cellind} & \text{otherwise},
%  \end{array} \right.
\end{align}
%for the $\cellind^{\text{th}}$ cell and the case $\spatialorder \geq 3$, that is piece-wise quadratic or higher-degree polynomials, so that the final rows of zeros in the first case indicates
%that the coefficients for the higher-order basis functions are set to zero for
%each component.
The absolute value and the inequality are applied componentwise. %The label ``scalar'' is used because the limiter is directly applied to each 
%scalar component of $\momentscollection{}$.
The function $\minmod{\cdot}$ is the standard minmod function applied componentwise, defined by
\begin{align}
\label{eq:minmod}
\minmod{a_1,a_2,a_3} &= \begin{cases}
 \operatorname{sign}(a_1) \min\{|a_1|,|a_2|,|a_3|\} & \text{if } 
 \operatorname{sign}(a_1) = \operatorname{sign}(a_2) = 
 \operatorname{sign}(a_3), \\
0 & \text{else}.
\end{cases}
\end{align}

The constant $\TVBconstant$ is a problem-dependent estimate of the second derivative, 
though it has to be noted that in \cite{Cockburn1989a} the authors did not find the 
solutions very sensitive to the value chosen for this parameter.


\subsection{Slope limiters and reconstructors}
\comment{bla}
\subsubsection{The minmod limiter}
Often-used due to its simplicity and small stencil is the following limiter
\begin{align*}
\slopelimitercf(\momentspolynomialmatrix{\cellind-\spatialorder},\ldots,\momentspolynomialmatrix{\cellind},\momentspolynomialmatrix{\cellind+\spatialorder})
= 
\left( \begin{array}{c}
\left( \momentspolynomialcoefficients{\cellind}{0} \right)^T \\
\minmod{\momentspolynomialcoefficients{\cellind}{1}, \momentspolynomialcoefficients{\cellind+1}{0} - \momentspolynomialcoefficients{\cellind}{0}, 
\momentspolynomialcoefficients{\cellind}{0} - \momentspolynomialcoefficients{\cellind-1}{0}}^T \\
                             (0, 0, \ldots , 0)\\
                             \vdots\\
                             (0, 0, \ldots , 0)
                            \end{array} \right)
\end{align*}
for the case $\spatialorder \geq 3$, that is piece-wise quadratic or higher-degree polynomials, so that the final rows of zeros in the first case indicates that the coefficients for the higher-order basis functions are set to zero for each component. As before, the minmod function is defined as in \eqref{eq:minmod}.

This limiter has the known disadvantage that it reduces the accuracy at smooth extrema for that it is mostly combined with the TVBM-corrected minmod indicator as in \secref{sec:TVBMminmod} which does not identify smooth extrema as troubled if the constant $\TVBconstant$ is chosen correctly. 

Note that there are generalizations of this indicator and limiter combination like in \cite{Krivodonova2007} which are not investigated here.

\subsection{WENO}
\comment{begin bla}
Here, the standard WENO reconstruction method given for example in \cite{Shu1998,Toro2009} is used.
For the unfamiliar reader, the method is introduced briefly in this section,
while a more detailed documentation\footnote{Most of the documentation and the code has been written by Jochen Kall.} and demo implementations of the
used reconstruction procedures can be found on the web page
\cite{AGTMWENOpage}. Note that the described techniques should in principle work with every accurate high-order polynomial reconstruction method.\\

Since it is not a priori clear what it means to do a polynomial reconstruction in space of a function in angle, the angular domain has to be discretized using the quadrature rule $\angularQuadrature$ (see \secref{sec:QRealizability}). Then, the following techniques can be applied at every quadrature point $\angularQuadratureNodes{\angularQuadratureIndex}$. For clarity of exposition, the time dependence is suppressed here.\\

Given polynomials of degree $\polydegree$, $\WENOpoly{\cellind}{\WENOind}(\cdot, \SCheight) \in \SpaceOfPolynomials{\polydegree}\left(\cell{\cellind}\right)$, $\WENOind = 0, 1, \ldots , \spatialorder$, each solving the interpolation problem
\begin{equation}
 \cellmean[\cellindvar]{\WENOpoly{\cellind}{\WENOind}(\z, \SCheight)} =  \distributioncellmean{\cellind}(\SCheight),
  \qquad \cellindvar \in \WENOstencil{\cellind}{\WENOind}{\spatialorder} := \{\cellind - \spatialorder + \WENOind, \ldots ,  \cellind + \WENOind - 1\},
\label{eq:interpolation}
\end{equation}
the WENO method then calculates coefficients $\WENOweights^{\pm}_{\cellind-\frac12, \WENOind}$
to form the weighted averages
$$
\WENOpoly{\cellind}{-\frac12}^\pm(\z, \SCheight) := \sum_{\WENOind = 0}^\spatialorder
 \WENOweights^{\pm}_{\cellind-\frac12, \WENOind} \WENOpoly{\cellind}{\WENOind}(\z, \SCheight).
$$

The set $\WENOstencil{\cellind}{\WENOind}{\spatialorder}$ is called the \emph{WENO stencil} of order $\spatialorder$ in cell $\cellind$ with shift $\WENOind$. The weights $\WENOweights^{\pm}_{\cellind-\frac12, \WENOind}$ are non-linear functions
of the cell-averages and reflect the smoothness of each polynomial $\WENOpoly{\cellind}{\WENOind}$. 
They are computed such that for smooth data the approximation order at the 
cell edge is maximized.
This gives an order $2 \spatialorder - 1$ approximation at the cell interface, while
the overall order in the interior of the cell is $\spatialorder$.

When at least one of the interaction coefficients $\absorption$ or
$\scattering$ is spatially dependent, it is necessary to specify the reconstruction
inside each cell. Thus it is essential to make a choice, because both $\WENOpoly{\cellind}{\mp \frac12}^\pm$
are order $\spatialorder$ reconstructions of the density $\ansatz$ in the $\cellind^{\text{th}}$ cell%
\footnote{
Some reconstruction methods, such as sub-cell WENO \cite{Cheng2013} or minmod \cite{Toro2009},
give only one polynomial reconstruction inside each cell, and so for these
methods such a choice would be unnecessary.
}.
\comment{end bla}

==> mesh.tex <==
\begin{center}
\includemovie[poster,toolbar,label=mesh.u3d,text=(mesh.u3d),
3Daac=7, 3Droll=0, 3Dc2c=0.000000 1.000000 0.000000, 3Droo=17.278794, 3Dcoo=0 0 0,3Dlights=CAD,]{\linewidth}
{\linewidth}{mesh.u3d}
\end{center}

